Borel Summability for Nonlinear Differential Systems on Characteristic Domains

We investigate singularly perturbed nonlinear complex differential systems of the form $\hbar \partial_x f = F (x, \hbar, f)$, where $\hbar$ is a small complex perturbation parameter. We give geometric and analytic conditions under which the formal perturbative solution associated with a fixed regular leading-order branch is locally uniformly Borel summable. This leads to an existence and uniqueness theorem of holomorphic solutions with prescribed perturbative expansion. We give an explicit triangular example and a self-contained application to the singularly perturbed Painlev\'e I equation.

==> src/project-preamble.tex <==
% Load this project's frozen house packages rather than globally installed copies.
% File substitution also covers dependencies requested internally by other packages.
\makeatletter
\declare@file@substitution{declare-style.sty}{src/declare-style.sty}
\declare@file@substitution{declare-style-notes.sty}{src/declare-style-notes.sty}
\declare@file@substitution{declare-maths.sty}{src/declare-maths.sty}
\declare@file@substitution{declare-text.sty}{src/declare-text.sty}
\declare@file@substitution{declare-tables-figures.sty}{src/declare-tables-figures.sty}
\declare@file@substitution{declare-theorems-notes.sty}{src/declare-theorems-notes.sty}
\declare@file@substitution{declare-bibliography.sty}{src/declare-bibliography.sty}
\makeatother

